A Declarative System for Optimizing AI Workloads

A long-standing goal of data management systems has been to build systems which can compute quantitative insights over large corpora of unstructured data in a cost-effective manner. Until recently, it was difficult and expensive to extract facts from company documents, data from scientific papers, or metrics from image and video corpora. Today's models can accomplish these tasks with high accuracy. However, a programmer who wants to answer a substantive AI-powered query must orchestrate large numbers of models, prompts, and data operations. For even a single query, the programmer has to make a vast number of decisions such as the choice of model, the right inference method, the most cost-effective inference hardware, the ideal prompt design, and so on. The optimal set of decisions can change as the query changes and as the rapidly-evolving technical landscape shifts. In this paper we present Palimpzest, a system that enables anyone to process AI-powered analytical queries simply by defining them in a declarative language. The system uses its cost optimization framework to implement the query plan with the best trade-offs between runtime, financial cost, and output data quality. We describe the workload of AI-powered analytics tasks, the optimization methods that Palimpzest uses, and the prototype system itself. We evaluate Palimpzest on tasks in Legal Discovery, Real Estate Search, and Medical Schema Matching. We show that even our simple prototype offers a range of appealing plans, including one that is 3.3x faster and 2.9x cheaper than the baseline method, while also offering better data quality. With parallelism enabled, Palimpzest can produce plans with up to a 90.3x speedup at 9.1x lower cost relative to a single-threaded GPT-4 baseline, while obtaining an F1-score within 83.5% of the baseline. These require no additional work by the user.

==> additionalworkloads.tex <==

\subsection{Additional Workloads}
% \matt{While SAPPs are an exciting new class of AI workloads which \system{} is designed to support, it also helps users optimize more ``traditional" systems such as ones using Retrieval Augmented Generation (RAG).}
Beyond SAPPs, there are a number of workloads which \system{} is well-suited to implement given its relational model and optimizer.

\noindent {\bf Document-driven discovery.} Organizations and individuals often wish to extract insights from sets of documents. For example, investors may wish to examine the footnotes of public US banks' SEC filings to see if they are at risk of a liquidation event. As another example, database researchers may try to process five years of VLDB and SIGMOD papers to extract specific metadata of interest (e.g., how the number of figures in accepted papers has varied over time).
\mjf{why isn't this a SAPP?  Seems to meet all the criteria}

Such tasks can easily be performed using \system{}. As shown previously in \autoref{fig:email} and \autoref{fig:examples}, users simply provide their source documents as an input {\tt Dataset} and define the metadata they wish to extract using their own {\tt Schema}. They may also perform additional post-processing on the extracted metadata following the schema conversion.

\noindent {\bf Multimodal integration.} Users often wish to integrate multiple datasources of differing modalities in order to enhance their ability to extract quantitative insights. For example, an insurance company may collect photos of a car crash along with police reports to help determine whether the driver they insure is at fault or not. Similarly, firefighters may collect streaming video data along with live weather maps to try to pinpoint the location of a brush fire. Once again, \system{} can assist users with creating AI systems for such workloads by allowing users to write simple {\tt Schemas} against each data modality to extract quantitative fields of interest.

\noindent {\bf Schema matching.}
To manage large collections of structured data from different sources often requires matching schemata across different tables.
For example, a medical researcher may wish to perform a large-scale study that requires integrating new patient data collected by previous field studies together with new experimental observations.
Or, environmental scientists may want to analyze climate change using historical data collected with different sensors across different geographical regions.
With the use of \system{}, users can write a simple specification of the target {\tt Schema} using natural language, and let \system{} automatically infer how to extract and match the existing attributes from all source datasets.

\noindent {\bf RAG systems.} The Retrieval Augmented Generation (RAG) architecture has rapidly become a first-class use case for neural models in enterprise settings. They are characterized by a two-stage process: first, a retrieval model is used to identify a set of candidate input documents, and then a generation model is used to produce a high-quality output based on the inputs. Even this dead-simple architecture exhibits performance, cost, and quality tradeoffs when the system designer decides how many documents to fetch from a vector database in Step 1. Too few means the LLM may not have relevant information it needs, while too many means the system performs unnecessary queries. \matt{\system{} is designed to optimize for these types of tradeoffs, thus supporting RAG applications is quite natural.}

\tim{I find it confusing that you mention RAG here. Everything else are use cases, RAG is a technique to achieve a particular goal, e.g., schema matching. For me it is on the same level as model selection, code generation, etc,. which are all tools/techniques to achieve a specific goal.} 
\mjf{I also think the above examples except for RAG could be considered SAPPs - no?  If so, then it is indeed interesting that the system (or at least the insights underlying it) could be used to support RAG, which as Tim says, seems different from the others.}

\system\ is designed to use the RAG architecture in two different ways. First, it can employ RAG-style methods as part of its query plan. For example, consider \st{a topic summarization program in \autoref{fig:extraction-example}} the use case of topic summarization over a set of documents. If the input document is larger than any available model's maximum token size, \system\ can decide, during synthesis of the convert operation, to use a RAG-style method to make the subtask manageable. That is, it may: (1) decompose the input text into smaller chunks, (2) choose chunks that are both relevant and will fit in the model's context size, then (3) generate the output summary using the selected chunks. This is a purely "internal" RAG approach, which is invisible to the user.

\matt{Matt: Re-reading the paragraph above made me realize that it pretty much summarizes Chunwei's input token reduction technique, because I doubt 95\% of users have documents which cannot fit in the context of the newest models. The more I think about it, the more I understand Tim's comment that, at least in our worldview, RAG is a token-reduction optimization which has quality and runtime tradeoffs as well. The key point we want to make is that PZ can optimize your RAG system for you --- but I think that falls outside of ``workloads" and maybe this text should go into ``optimizations"? Perhaps we should reframe this subsection as illustrating how ``traditional workloads" can be represented as SAPPs. I.e. ``document-driven discovery is a SAPP where the input is ... multimodal integration is a SAPP which focuses on the extraction of structured fields from ... Schema matching is a SAPP in which ..." }

The system can also support "external" RAG applications in which the user has an external data store of documents. \system\ allows users to define their own datasources, and can use these sources as part of the query plan. We understand from talking with industrial contacts that one of the primary engineering challenges encountered when building RAG systems is managing the inevitable quality/runtime tradeoffs. For example, how many 
documents should be returned by the vector database in response to a query? Too many, and the system is unnecessarily slow; too few, and the system yields bad results. This kind of tradeoff is exactly what \system\ was designed to handle: we are currently working on an extension that will allow \system\ to optimize these external RAG database queries.

% \noindent {\bf Database Administration}


% Older content:

% \noindent {\bf }

% Functionalities we wish to highlight:
% \begin{itemize}
%     \item \textbf{Queries over text / PDFs}
%     \begin{itemize}
%         \item Searching Enron emails for ref. to Special Purpose Entities (SPEs) (i.e. fraud)
%         \item Matching investment hypothesis to companies' public filings
%     \end{itemize}
%     \item \textbf{Queries over images}
%     \begin{itemize}
%         \item Semantic search over image repos (``find a photo of my dog playing in the snow")
%         \item Satellite image classification (Amazon deforestation)
%         \item Stream classifiers (e.g. imagine having an Amber Alert which only requires updating the Alert prompt rather than re-training an image classifier)
%     \end{itemize}
%     \item \textbf{Multi-modal queries}
%     \begin{itemize}
%         \item Fake Amazon products \& reviews
%         \item Search over video / audio + transcription
%         \item Investment hypothesis (PDF + stock time-series data)
%     \end{itemize}
%     \item \textbf{Queries which require using RAG}
%     \begin{itemize}
%         \item Understanding my tax liability (querying IRS docs + tax law)
%         \item (Possibly investment hypothesis example; we may need to pre-process PDFs and perform RAG over their contents)
%     \end{itemize}
% \end{itemize}

==> system.tex <==

%We have implemented the \st{{\bf Plan Scoring} module} \matt{cost optimizer's {\bf Plan Scoring} module (discussed in \autoref{sec:planning})} through a number of techniques. The prototype contains a \st{database} \matt{catalog} of observations around model performance, cost, and quality collected from academic papers and service-published statistics. We use this \st{database} \matt{information}, along with \st{input data} statistics \matt{related to the size of the input relation}, to compute a very rough \matt{initial} score for each candidate plan. 

%The system also collects statistics about every plan during execution. If the plan is expected to run long enough, we will process a few inputs using preliminary "probe plans" that exist primarily to collect performance statistics. After the brief initial probe period, the system can then use these statistics to improve its estimates of the physical plan(s) it is executing \textbf{\textit{and}} other plans which it has not yet executed. For example, the distribution of source records' token lengths is useful information regardless of which model is chosen. On the other hand, some elements of cost and runtime cannot be estimated without switching physical plans.  



%This resembles a multi-armed bandit problem, where it may be beneficial to try multiple plans near the beginning of program execution in order to find the optimal plan, although we do not pursue this strategy in the current prototype.
%One particularly difficult challenge is estimating the quality of an operator's --- and a plan's --- generated outputs.  Currently we use both historical data and compare different models' outputs against those of a "champion" model that is known to have good quality (but which might have other unappealing characteristics).

%\system{} takes a user-written program and compiles it down to a (set of) physical plan(s) inside of its {\tt pz.Execute} class. In order to select one or more of the physical plans to execute, users must also provide a policy specifying their priorities regarding quality and cost, i.e., where they would like to operate on the pareto-frontier of plans in terms of the tradeoff between quality and cost. For example, a policy can minimize cost, maximize quality, or maximize the harmonic mean of cost and quality. Different policies may also allow the system to execute multiple plans with similar cost-quality tradeoffs in parallel to further maximize throughput.


%A crucial element of the \system{} system is its ability to re-optimize the physical plan(s) as it is executing a user's AI program. In brief, as \system{} executes a physical plan, it records the time and cost of each operation on a per-record basis. 


%This degree of caching presents two challenges. First, storing every intermediate result means that \system{} can quickly exceed the memory limits of even memory-optimized cloud compute instances. This implies that a significant portion of the cache must be spilled to disk. Second, for convert operations --- especially ones using prompt-level optimizations such as DSPy --- the continuous learning of an optimal (set of) prompt(s) means that the results of a convert operation may vary with each execution.

%Due to the orders of magnitude difference between the throughput of LLMs and every other component of the \system{} system, we are able to make unusual, yet reasonable design choices to mitigate these challenges. First, we recognize that reading from disk (or even remote storage) still provides orders of magnitude higher throughput (\textcolor{blue}{and cheaper cost}) than invoking an LLM to regenerate an output. Thus, spilling an entire history of intermediate results and reading them from disk can be a pareto-optimal design decision (on throughput and cost) depending on the user's workload. Second, for many workloads, small improvements in output generation quality may not be worth the cost of regenerating an entire \texttt{Dataset}. For example, if a user wants an estimate of an aggregate, it may be perfectly fine to re-use a cached computation even if a prompt optimizer learned an improved prompt. In each of these situations, the \system{} optimizer can decide whether to read from its cache or recompute an intermediate result based on the user workload, the optimizer's estimate of the cost vs. quality tradeoff, and the user's preferred policy (e.g., to minimize cost or maximize quality).

